Study of Unsteadiness due to 3-D Shock-Boundary Layer Interaction in Flow over a Square-faced Protuberance

The dynamics of shock-induced unsteady separated flow past a three-dimensional square-faced protuberance is investigated through wind tunnel experiments. Time-resolved schlieren imaging and unsteady surface pressure measurements are the diagnostics employed. Dynamic Mode Decomposition (DMD) of schlieren snapshots, and analysis of spectrum and correlations in pressure data are used to characterize and resolve the flow physics. The mean shock foot in the centreline is found to exhibit a Strouhal number of around 0.01, which is also the order of magnitude of the Strouhal numbers reported in the literature for two-dimensional shock-boundary layer interactions. The wall pressure spectra, in general, shift towards lower frequencies as we move away from (spanwise) centreline with some variation in the nature of peaks. The cross-correlation analysis depicts the strong dependence of the mean shock oscillations to the plateau region, and disturbances are found to travel upstream from inside the separation bubble. Good coherence is observed between the spanwise mean shock foot locations till a strouhal number of about 0.015 indicating that the 3-D shock foot largely moves to-and-fro in a coherent fashion.

==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time-delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.


\end{thebibliography}


